BIM-SLAM: Integrating BIM Models in Multi-session SLAM for Lifelong Mapping using 3D LiDAR

While 3D LiDAR sensor technology is becoming more advanced and cheaper every day, the growth of digitalization in the AEC industry contributes to the fact that 3D building information models (BIM models) are now available for a large part of the built environment. These two facts open the question of how 3D models can support 3D LiDAR long-term SLAM in indoor, GPS-denied environments. This paper proposes a methodology that leverages BIM models to create an updated map of indoor environments with sequential LiDAR measurements. Session data (pose graph-based map and descriptors) are initially generated from BIM models. Then, real-world data is aligned with the session data from the model using multi-session anchoring while minimizing the drift on the real-world data. Finally, the new elements not present in the BIM model are identified, grouped, and reconstructed in a surface representation, allowing a better visualization next to the BIM model. The framework enables the creation of a coherent map aligned with the BIM model that does not require prior knowledge of the initial pose of the robot, and it does not need to be inside the map.

==> 00_Template/ECPPM_main.tex <==
%narms.tex, an example driver file for Balkema documents.

%use the following for A4 paper:

%\documentclass[12pt,a4paper,twocolumn,fleqn]{narms}

% packages needed
\usepackage{subfigure}
\usepackage{epsfig}
\usepackage{timesmt}

% add here more packages based on the document format


% setting math equation indent from left 0pts
\mathindent=0pt%

% use this for chicaco style reference
% Author references
% IMPORTANT: Author wants to format references in chicaco style Author must use BiBTex
% IMPORTANT: Author wants to format numbered references remove chicaco style file and \bibliographystyle{chicaco}

\usepackage{00_Template/chicaco}

%\documentclass{scrartcl}
\begin{document}

\title{Occupancy Grid Map to Pose Graph-based Map: BIM-based 2D-LiDAR localization for lifelong navigation in changing and dynamic environments}
\author{{M.A. Vega Torres \& 
A. Braun 
\& A. Borrmann} \\
{\aff{Chair of Computational Modeling and Simulation}} \\
{\aff{Technical University of Munich, Munich, Germany}
}}
%\\


%{\authornext{R. Schielen}}\\
%{\aff{Department of Water Engineering and Management}} \\
%{\aff{University of Twente, Enschede, The Netherlands.}}}

\date{}% No date.
\input{01_Content/00_abstract}


\maketitle

%% Page limit 8 -> including references (i.e. in total 7 pages)
% 1: Intro
% 2: Theory
% 3: Related work
% 4: Methodology
% 5: Experiments 
% 6: Results and analysis
% 7: Conclusions
% 8: Future work and references

% \input{01_Content/01_Introduction.tex}
% \input{01_Content/02_Theoretical_Background}
% \input{01_Content/03_RelatedResearch.tex}
% \input{01_Content/04_Methodology.tex}
% \input{01_Content/05_Experiments.tex}
% \input{01_Content/06_Results_and_Analisys.tex}
% \input{01_Content/07_Discussion.tex}
% \input{01_Content/08_Conclusions.tex}





\shortcite{cg00}
% Now, periodic solutions of the type (\ref{persol}) need not to be
% stable. The stability can be studied by considering perturbations
% of $P$ and $\Theta$:
% \begin{equation}
% A=[ P+\rho(X,T)] \exp [ i (\Theta+\theta(X,T))]


\bibliographystyle{00_Template/chicaco}
\bibliography{03_References/a4sample}

\end{document}


==> 00_Template/ISARC_Instruction_camera-ready.tex <==
%\documentclass[a4paper, 10pt, twocolumn, twoside]{article}

\usepackage{ISARC}

\usepackage{lscape}
\usepackage{hologo}



\begin{document}

 % Do not change the following line
\linespread{0.5}

\title{Instructions to authors for the preparation of \\ISARC manuscripts}

\author{Author1FirstName Author1LastName$^{1}$ and Author2FirstName Author2LastName$^2$}

\affiliation{
$^1$School of ..., University of ..., Country\\
$^2$School of ..., University of ..., Country
}

\email{
\href{mailto:e.author1@aa.bb.edu}{author1@aa.bb.edu}, 
\href{mailto:e.author1@aa.bb.edu}{author2@cc.dd.edu}
}


% Do not change the following three lines
\maketitle 
\thispagestyle{fancy} 
\pagestyle{fancy}



\begin{abstract}
This document sets out the requirements for preparing manuscripts for the ISARC.
It is essential that all manuscripts conform to these instructions. 
Note that this document contains both general instructions and structures specific to the preparation of manuscripts using \hologo{LaTeX}.
For instructions on how to prepare manuscripts using MS Word, please use the MS Word template.
\end{abstract}

\begin{keywords}
Instructions; Formatting; Authors; ISARC
\end{keywords}


\section{Introduction}
\label{sec:Introduction}

This \hologo{LaTeX} template and the instructions it contains will enable you to prepare your manuscript in an electronic format (pdf), ready for submission and peer review. It is therefore essential that these instructions be carefully followed.

Your manuscript must be submitted to our online peer-review management system.

The Manuscript should not exceed 8 pages in length, including text, figures, tables, and references. Electronic file should not exceed 5 megabytes.

Authors are responsible for ensuring the accuracy of all information contained in their manuscripts (e.g., proper names of organizations, data and findings, references, etc.). Manuscripts must be prepared in proper English. SI units or acceptable metric equivalents must be used throughout.

\section{Preparation of the manuscript}
\label{sec:Preparation}


%When prepared in Word, the manuscript must be submitted in PDF format. 
You can prepare your manuscript with \hologo{LaTeX} by using the Overleaf template at \url{https://www.overleaf.com/latex/templates/isarc-paper-template/cdfwbxsghpyv}. You can alternatively download the source code from the Overleaf template and use it in another editor.

The rest of the manuscript details the formatting requirements for your submission.

Note that this document is a template, and thus already implements all the specified formatting. 
Therefore, if you use it to write your manuscript, and utilize the same commands, then your manuscript will naturally have the correct format. 



\subsection{Page Size and Layout}

Your manuscript must be prepared for A4-size (210 x 297 mm) paper. 
Use the margin settings specified in Table 1 and do not number the pages of the paper.
The \hologo{LaTeX} template already implements those margins.

\begin{table}[htb!]
\centering
\caption{Manuscript margins}
\begin{tabular}{cc}
\hline
Margin	&A4 (210 x 297 mm)\\
\hline
Top		&3.5 cm\\
Bottom	&3.5 cm\\
Left	&2.5 cm\\
Right	&2.0 cm\\
\hline
\end{tabular}
\end{table}


\subsubsection{Headers and footers}

Do not add anything in the footers or headers, even page numbers.

\subsection{Type Style and Spacing}

All text must use the Times New Roman font.
This \hologo{LaTeX} template already implements this.

\subsubsection{Title Page}

The title page of your manuscript is illustrated by the first page of these instructions. The title page must not exceed one (1) page in length. It contains:
\begin{enumerate}[noitemsep]
    \item The title of the paper in bold 18 points Times New Roman, centered with first letters in capitals.
    \item The authors’ names, separated from the title by a one blank line, are centered and in size 11, bold Times New Roman.
    \item The authors’ affiliations and addresses are put immediately below the names, centered and single-spaced, in size 10.
    \item 	Email addresses are inserted below the affiliations, also in size 10.
\end{enumerate}

This template already implements all these requirements. Simply use the commands \verb|\title{}|, \verb|\author{}|, \verb|\affiliation{}| and \verb|\email{}| as illustrated here.

\subsubsection{Body of paper}

The body of the paper follows the front matter. It contains two columns (with 0.5cm separation) and begins with:
\begin{itemize}[noitemsep]
    \item The major heading “Abstract –”, in bold.
    \item 	The body of the abstract, not to exceed 250 words in length, in bold Times New Roman, fully justified, the first line is indented.
    \item The major heading “Keywords –” in bold, separated from the last line of the abstract by one blank line.
    \item The list of keywords, not to exceed ten (10) words, in bold Times New Roman, left justified, indented, and separated by commas. Please add those keywords that you would use if you were searching for your paper. 
    
\end{itemize}
The main text of the paper begins after. Separate sections of the main text in accordance with the Headings guidelines below

This template already implements all these requirements. Simply use the environments \verb|abstract| and \verb|keywords| as illustrated in this template.

\subsubsection{Headings}

All headings must be in black and in bold face. The manuscript will typically have maximum three levels of headings maximum: Level 1, Level 2, and Level 3. Level-1 headings (e.g. Introduction, Background, Discussion, Conclusions, Acknowledgments, References) have font size 12; Level-2 headings have font size 11; and Level-3 headings have font size 10. 

Words in the headings should be all lower case, except the first letter of the first word which must start with a capital letter. The headings are positioned at the left margin. They are numbered in the form "1." for Level-1 headings, "1.1." for Level-2 headings, and "1.1.1" for Level-3 headings.

The commands \verb|\section{}|, \verb|\subsection{}| and \verb|\subsubsection{}| employed in this template implement the requirements above for headings Level 1, 2 and 3.
Note that you may also use the command \verb|\paragraph{}|, if this suits better your needs.

\subsubsection{Text}

Text paragraphs are single-spaced and fully justified, with the first line indented 0.5 cm. Do not use blank lines between paragraphs unless you feel it important to really highlight a change of topic (in such a case, you should also consider using sub-headings).

Note that, to start a new paragraph in \hologo{LaTeX}, simply leave a blankline in the \verb|.tex| file. 

\subsubsection{Lists}

\begin{enumerate}[noitemsep]
\item
Numbered lists should be presented using the environment \verb|enumerate| like in this example. 
This environment applies the numbering and defines the format and spacing automatically. 
\item 
Add the option \verb|[noitemsep]| to the environment to have no additional space between numbered list items.
\end{enumerate}

\begin{itemize}[noitemsep]
\item
Bulleted lists should be presented using the environment \verb|itemize| like in this example. 
This environment applies the numbering and defines the format and spacing automatically. 
\item 
Add the option \verb|[noitemsep]| to the environment to have no additional space between bulleted list items.
\end{itemize}

Note that the two list above were generated using the environments and options described within them.

\subsubsection{Footnotes}

Do not use footnotes. Incorporate all required information in the body of the paper.

\subsubsection{Equations and symbols}

Simple mathematical expressions and sub- and super-scripted characters, such as $SO_4^2$, are inserted in the text. 
Do not embed equations as an image.
\hologo{LaTeX} is valued particularly for its performance in handling equations and symbols.

Equations are placed on separate lines, centered and numbered consecutively in parentheses at the right-hand margin. 
A blank line precedes and follows each equation.

To achieve this, simply use the environment {\it `equation'} as in the examples below.

%For reactions, preferably use the Times New Roman (normal text) arrow, Equation (\ref{eq_1}), but an equal sign may be substituted, Equation (\ref{eq_2}). 
%Use a dash rather than a hyphen for the minus sign, Equation (\ref{eq_3}). A good way to achieve the formatting above is to use a table (with invisible borderlines) with two columns, the right column being used for the numbering. The equations below are formatted like that.

\begin{equation}\label{eq_1}
ZnS + 3/2O_2 \rightarrow ZnO + SO_2
\end{equation}
\begin{equation}\label{eq_2}
ZnS + 3/2O_2 = ZnO+ SO_2
\end{equation}
\begin{equation}\label{eq_3}
E = 1.23 - 0.06 pH
\end{equation}

The nomenclature and units for symbols must be defined in the text. Alternatively, where the number of symbols is large, a special Section  \textbf{Nomenclature} should be used at the end of the manuscript.

\subsection{Figures}

Figures should appear as close as possible to their first citation. 
They should be numbered consecutively using Arabic numerals and their title should be centered below the figure.

Figures, such as graphs and diagrams, should be embedded in vector format (e.g.\verb|.eps|, \verb|.pdf| or \verb|.emf|), if at all possible. 
Otherwise, figures such as pictures should be with high resolution (300 dpi) when published at 100\% (e.g., images at 72 dpi are in reality 25\% of the required resolution).

For example, Figure 1 in this manuscript is embedded as a picture with high resolution (but, ideally, such graph should be prepared and embedded in vector format).
Lines and lettering must be large enough (minimum 0.35pt thickness) to remain clearly legible when printed at 100\%. 
For maps and similar figures, be sure to place a scale marker on the picture or photograph. 
Color is preferable; any grayscale figure requires sharp contrast. 
Please, refrain from using frames around figures, or using shaded backgrounds.
Figures can significantly increase the size of the electronic file. Excessively large files tend to complicate and slow down the editing process. Therefore, you must make every effort to reduce the size of the electronic files of your figures. Embedding figures in vector format, as mentioned above, can significantly reduce file size while simultaneously enhancing figure quality.

The caption should be formatted with the word `Figure' followed by the figure number, a period, a space, and the title. 
Each figure and caption should be separated from the adjacent text with one blank line. 
To achieve all this formatting, simply use the environment \verb|figure| as in Figure~\ref{fig_1}. 

A figure too wide to fit in one column may be placed across the width of the page (i.e. between the margins) by using the environment \verb|figure*|.
A figure too wide to fit between the margins may be placed in landscape orientation (sideways format), on a page by itself, with the bottom of the figure to the right of the page.
To achieve this, embed the environment \verb|figure| within an environment \verb|landscape|.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.48\textwidth]{ISARC_ExampleFigure.eps}
    \caption{Effect of iron concentration on the amount of precipitate formed during hydrolytic precipitation from waste processing solutions}
    \label{fig_1}
\end{figure}




\subsection{Tables}

Tables should appear as close as possible to their first citation. 
They should be numbered consecutively using Arabic numerals and their title should be centered above the table.

The caption should be formatted with the word `Table ' followed by a character space, the table number, a period, another character space, and the title. 
Separate each table from the adjacent text with one blank line.
See Table~\ref{tab_1} for example.

Table-wide lines (horizontal 0.5 point thickness) separate the title from the column headings, the column headings from the body of the table, and the table from the following text. 
Avoid vertical lines and avoid the use of horizontal lines between the various rows of data. 

Text in the tables should have the same size as the main text, but not be indented and with space before and after it. 
Table~\ref{tab_1} shows a good example.
A table too wide to fit in one column may be placed across the width of the page (i.e. between the margins) by using the environment \verb|table*|. 
A table too wide to fit between the margins may be placed in landscape orientation (sideways format), on a page by itself, with the bottom of the figure to the right of the page.
To achieve this, embed the environment \verb|table| within an environment \verb|landscape|.

\begin{table}[!htb]
    \centering
    \caption{Electron microprobe analyses of sphalerite grains in the Kidd Creek ``C'' concentrate}
    \label{tab_1}
    \begin{tabular}{ccc}
    \hline
    Element & Average(wt \%) & Range(wt\%)\\
    \hline
    Zn	&60.8	&59.6 - 63.3\\
    Fe	&5.82	&3.54 - 6.95\\
    Cd	&0.30	&0.12 - 0.42\\
    S	&3.31	&33.6 - 33.5\\
    \hline
    \end{tabular}
\end{table}


\subsection{Cross-referencing headings, numbered equations, figures and tables}

Refer to a figure as `Figure X', not using its relative position.
For achieving this effectively, use the command \verb|\label{}| within the environment \verb|figure| to label each figure, and then use the command \verb|\ref{}| in the text to refer to the label.

The same guidance applies to Tables and Equations, as well as Headings.
In the case of headings, the command \verb|\label{}| must be declared right after the heading commands (e.g. after the command \verb|\section{}|).

Note that all the figures, tables, equations and the main headings in this template all have a label and are referred to in the text using the command \verb|\ref{}|.


\subsection{References}

References to the literature should be cited in the main text with an Arabic number in square brackets \cite{Ha_2012}. 
References should then appear in cited order at the very end of your paper in the Section \textbf{References}. 
Start each reference on a new line with its number in square brackets \cite{Ha_2012}. 
Citation formats are given below for: a journal article \cite{Ha_2012}, conference paper \cite{Kwok_2012}, book \cite{Book}, and a website \cite{Website}.

The formatting of the references is done automatically by the \hologo{LaTeX} template.
All you need to do is add your references in the ISARC.bib Bibtex file and cite the papers in the text using the command \verb|\cite{}| (as well as \verb|\citet{}|).

Within the Bibtex file, please ensure that all references that have a DOI actually include it. It will then appear in the compiled references.



\bibliography{ISARC}

\end{document}


==> 00_Template/howToCitate.tex <==
%  \cite{key}
%    which produces citations with full author list and year.
%    eg. (Brown 1978; Jarke, Turner, Stohl, et al. 1985)

%  \citeNP{key}
%    which produces citations with full author list and year, but without
%    enclosing parentheses:
%    eg. Brown 1978; Jarke, Turner & Stohl 1985

%  \citeA{key}
%    which produces citations with only the full author list.
%    eg. (Brown; Jarke, Turner & Stohl)

%  \citeANP{key}
%    which produces citations with only the full author list, without
%    parentheses eg. Brown; Jarke, Turner & Stohl

%  \citeN{key}
%    which produces citations with the full author list and year, but
%    can be used as nouns in a sentence; no parentheses appear around
%    the author names, but only around the year.
%      eg. Shneiderman (1978) states that......
%    \citeN should only be used for a single citation.

%  \shortcite{key}
%    which produces citations with abbreviated author list and year.

%  \shortciteNP{key}
%    which produces citations with abbreviated author list and year.

%  \shortciteA{key}
%    which produces only the abbreviated author list.

%  \shortciteANP{key}
%    which produces only the abbreviated author list.

%  \shortciteN{key}
%    which produces the abbreviated author list and year, with only the
%    year in parentheses. Use with only one citation.

%  \citeyear{key}
%    which produces the year information only, within parentheses.

%  \citeyearNP{key}
%    which produces the year information only.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  All this stuff is from modifying the article.cls for Balkema
%%%  specifications.

%\title{...}
%\author{...}
%use \aff for author affiliations
% use \authornext for from second author
% empty line space between multiple authors
%\abstract{...}
%\maketitle{}

%%%%%%% Style for TABLES
% insert tabular command inside \tabletext{} this will produce tables in 10pts

==> 01_Content/02_Theoretical_Background.tex <==

\section{Theoretical background}
\label{ltheory}
%% Not used here

==> 01_Content/06_Results_and_Analisys.tex <==
\section{Results and discussion}
\label{chap:results}


% Table of quantitative results
\input{04_Tables/results1}






